The Conversion of CESR to Operate as the Test Accelerator, CesrTA, Part 1: Overview

Cornell's electron/positron storage ring (CESR) was modified over a series of accelerator shutdowns beginning in May 2008, which substantially improves its capability for research and development for particle accelerators. CESR's energy span from 1.8 to 5.6 GeV with both electrons and positrons makes it ideal for the study of a wide spectrum of accelerator physics issues and instrumentation related to present light sources and future lepton damping rings. Additionally a number of these are also relevant for the beam physics of proton accelerators. This paper outlines the motivation, design and conversion of CESR to a test accelerator, CesrTA, enhanced to study such subjects as low emittance tuning methods, electron cloud (EC) effects, intra-beam scattering, fast ion instabilities as well as general improvements to beam instrumentation. While the initial studies of CesrTA focussed on questions related to the International Linear Collider (ILC) damping ring design, CesrTA is a very flexible storage ring, capable of studying a wide range of accelerator physics and instrumentation questions. This paper contains the outline and the basis for a set of papers documenting the reconfiguration of the storage ring and the associated instrumentation required for the studies described above. Further details may be found in these papers.

==> FrontMatter/def_affiliations.tex <==
\def\cornell{Cornell Laboratory for Accelerator-based Sciences and Education, Cornell University, Ithaca, NY, 14850, U.S.A.\ }
\def\americanriver{American River College, Sacramento, CA 95841, U.S.A.\ }
\def\anl{Argonne National Laboratory, Argonne, IL 60439, U.S.A.\ }
\def\aussynch{Australian Synchrotron, Clayton, 3168, Australia.\ }
\def\bnl{Brookhaven National Laboratory, Upton, NY 11973, U.S.A.\ }
\def\calpoly{California Polytechnic State University, Physics Department, San Luis Obispo, CA 93407, U.S.A.\ }
\def\carleton{Carleton University, Department of Physics, Ottawa, Ontario, K1S 5B6, Canada\ }
\def\carnegiemellon{Carnegie Mellon University, Department of Physics, Pittsburgh, PA, 15389, U.S.A.\ }
\def\cern{CERN, CH-1211 Gen\`{e}ve 23, Switzerland\ }
\def\clarkson{Clarkson University, Department of Physics, Potsdam, NY 13699, U.S.A.\ }
\def\cockroft{Cockroft Institute, Warrington, Cheshire, U.K.\ }
\def\dimtel{Dimtel, Inc., San Jose, CA 95124, U.S.A.\ }
\def\fnal{Fermi National Accelerator Laboratory, Batavia, IL 60510, U.S.A.\ }
\def\grovecity{Grove City College, Physics Department, Grove City, PA 16127, U.S.A.\ }
\def\harvard{Harvard University, Department of Physics, Cambridge, MA 02138, U.S.A.\ }
\def\harveymudd{Harvey Mudd College, Department of Physics, Claremont, CA 91711, U.S.A.\ }
\def\indiana{Indiana University, Department of Physics, Bloomington, IN 47405, U.S.A.\ }
\def\infn{Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, 00044 Frascati, Italy\ }
\def\kek{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan\ }
\def\lanl{Los Alamos National Laboratory, Los Alamos, NM 87544, U.S.A.\ }
\def\lbnl{Lawrence Berkeley National Laboratory, Berkeley, CA 94270, U.S.A.\ }
\def\loyola{Loyola University, Department of Physics, Chicago, IL, 60626, U.S.A.\ }
\def\postech{Postech, Department of Physics, Pohang, Gyeongbuk 790-784, R.O.K.\ }
\def\purdue{Purdue University, Department of Physics, West Lafayette, IN 47907, U.S.A.\ }
\def\slac{SLAC National Accelerator Laboratory, Menlo Park, CA 90425, U.S.A.\ }
\def\syracuse{Syracuse University, Department of Physics, Syracuse, NY 13244, U.S.A.\ }
\def\technion{Technion-IIT, Department of Electrical Engineering, Haifa, 32000, Israel\ }
\def\techx{Tech-X Corporation, Boulder, CO, 80303, U.S.A.\ }
\def\tufts{Tufts University, Department of Physics and Astronomy, Medford, MA 02155, U.S.A.\ }
\def\utah{University of Utah, Department of Physics and Astronomy, Salt Lake City, UT 84112, U.S.A.\ }


==> FrontMatter/definitions.tex <==
% 
%  File:  PhaseI_Report/definitions.tex
%
%  Special definitions used throughout the document
%

% ------------ Set section numbering depth ------------ 
\setcounter{secnumdepth}{3}

% ------------ Some common definitions ------------ 

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{exercise}{Exercise}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{warning}{Warning}

\def\grad{ \mbox{grad}}
\def\curl{ \mbox{curl}}
\def\div{ \mbox{div}}
\def\U{\ensuremath {\cal U}}
\def\S{\ensuremath {\cal S}}
\def\V{\ensuremath {\cal V}}
\def\R{\ensuremath {\cal R}}
\def\tr{\ensuremath {\mbox{tr}}}


% ------------ Custom definitions for this report ------------ 

% Custom chapter heading command
\newcommand{\mychapter}{Chapter \thechapter:}

% Define a custom \cesrta text string  (requires the relsize package)
\def\cesrta{{C{\smaller[2]ESR}TA}}
%\def\cesrta{CESRTA}

% Affilliations
\def\cornell{Cornell Laboratory for Accelerator-based Sciences and Education, Cornell University, Ithaca, NY, 14850, U.S.A.\ }
\def\americanriver{American River College, Sacramento, CA 95841, U.S.A.\ }
\def\anl{Argonne National Laboratory, Argonne, IL 60439, U.S.A.\ }
\def\aussynch{Australian Synchrotron, Clayton, 3168, Australia.\ }
\def\bnl{Brookhaven National Laboratory, Upton, NY 11973, U.S.A.\ }
\def\calpoly{Physics Department, California Polytechnic State University, San Luis Obispo, CA 93407, U.S.A.\ }
\def\carleton{Department of Physics, Carleton University, Ottawa, Ontario, K1S 5B6, Canada.\ }
\def\carnegiemellon{Department of Physics, Carnegie Mellon University, Pittsburgh, PA, 15389, U.S.A.\ }
\def\cern{CERN, CH-1211 Gen\`{e}ve 23, Switzerland.\ }
\def\clarkson{Department of Physics, Clarkson University, Potsdam, NY 13699, U.S.A.\ }
\def\cockroft{Cockroft Institute, Warrington, Cheshire, U.K.\ }
\def\dimtel{Dimtel, Inc., San Jose, CA 95124, U.S.A.\ }
\def\fnal{Fermi National Accelerator Laboratory, Batavia, IL 60510, U.S.A.\ }
\def\grovecity{Physics Department, Grove City College, Grove City, PA 16127, U.S.A.\ }
\def\harvard{Department of Physics, Harvard University, Cambridge, MA 02138, U.S.A.\ }
\def\harveymudd{Department of Physics, Harvey Mudd College, Claremont, CA 91711, U.S.A.\ }
\def\indiana{Department of Physics, Indiana University, Bloomington, IN 47405, U.S.A.\ }
\def\infn{Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, 00044 Frascati, Italy.\ }
\def\kek{High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan.\ }
\def\lanl{Los Alamos National Laboratory, Los Alamos, NM 87544, U.S.A.\ }
\def\lbnl{Lawrence Berkeley National Laboratory, Berkeley, CA 94270, U.S.A.\ }
\def\loyola{Department of Physics, Loyola University, Chicago, IL, 60626, U.S.A.\ }
\def\postech{Department of Physics, Postech, Pohang, Gyeongbuk 790-784, R.O.K.\ }
\def\purdue{Department of Physics, Purdue University, West Lafayette, IN 47907, U.S.A.\ }
\def\slac{SLAC National Accelerator Laboratory, Menlo Park, CA 90425, U.S.A.\ }
\def\syracuse{Department of Physics, Syracuse University, Syracuse, NY 13244, U.S.A.\ }
\def\technion{Department of Electrical Engineering, Technion-IIT, Haifa, 32000, Israel.\ }
\def\techx{Tech-X Corporation, Boulder, CO, 80303, U.S.A.\ }
\def\tufts{Department of Physics and Astronomy, Tufts University, Medford, MA 02155, U.S.A.\ }
\def\utah{Department of Physics and Astronomy, University of Utah, Salt Lake City, UT 84112, U.S.A.\ }

% Partial derivative definitions (GFD)

\newcommand{\der}[2]{\frac{d {#1}}{d {#2}}}
\newcommand{\dder}[2]{\frac{d^2 {#1}}{d {#2}^2}}
\newcommand{\pder}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\ppder}[3]{\frac{\partial^2 {#1}}{\partial {#2}\,\partial {#3}}}
\newcommand{\pdder}[2]{\frac{\partial^2 {#1}}{\partial {#2}^2}}


% Chapter 4 definitions (MAF)
\newcommand{\deltamax} {\delta_\text{max}}
\newcommand{\deltaeff} {\delta_\text{eff}}
\newcommand{\Emax} {E_\text{max}}
\newcommand{\etaeff} {\eta_\text{eff}}
\newcommand{\ndot} { {\dot n}}
\newcommand{\ndote} { {\dot n}_e}
\newcommand{\xv} {{\bf x}}
\newcommand{\vv} {{\bf v}}
\newcommand{\sigx} {\sigma_x}
\newcommand{\sigy} {\sigma_y}
\newcommand{\sigz} {\sigma_z}
\newcommand{\sigt} {\sigma_t}
\newcommand{\betabar} {{\bar\beta}}
\newcommand{\rhobar} {{\bar\rho}}
\newcommand{\Ebar} {{\bar E}}
\newcommand{\lambdabar} {{\bar\lambda}}
\newcommand{\lmbe} {\lambdabar_e}
\newcommand{\lmbb} {\lambdabar_b}

\newcommand{\Nb} {N_b}
\newcommand{\Nbth} {N_{b,th}}
\newcommand{\intl}[2] {\int\limits_{#1}^{#2}} %% example:\intl{0}{\infty}
\newcommand{\ttt}[1] {\times10^{#1}}
\newcommand{\dotprod} {{\raisebox{-.7mm}{\hspace{.4mm}\LARGE$\cdot$\hspace{.4mm}}}}
\newcommand{\rar} {\rightarrow}
\newcommand{\lrar} {\leftrightarrow}
\newcommand{\abs}[1] {\left|{#1}\right|}
\newcommand{\absfix}[1] {|{#1}|}
\newcommand{\invpt}[1] {{\rule[#1]{0pt}{0pt}}} %invisible, zero-width point at height #1
\newcommand{\separate}[1] {\noalign{\hbox{\vspace{#1}}}}
\newcommand{\Dtr} {\Delta_{tr}}
\newcommand{\beq} {\begin{equation}}
\newcommand{\eeq} {\end{equation}}


%---------------------- Custom Title Page Definition -------------
\makeatletter
\def\maketitle{%
  \null
  \thispagestyle{empty}%
%  \vfill
  \vskip 2 in
  \begin{center}\leavevmode
    \normalfont
    {\huge \@title\par}%
    \vskip 1cm
    {\Large \emph{Editors:} \hskip0.2in \editors \par}%
    \vskip 1cm
    {\Large \@date\par}%
  \end{center}%
  \vfill
  \newpage
    \thispagestyle{empty}%
    \begin{center}\leavevmode
    \normalfont
    {\flushleft \Large \emph{Program Contributors:} \par}%
    \vskip 0.5cm
    {\large \@author \par}%
  \end{center}%
  \vfill
  \null
  \cleardoublepage
  }
\makeatother


% ------------------- Fancy Header Styles -----------------------------

% Define the fancy pagestyle
\pagestyle{fancy}
%\renewcommand{\chaptermark}[1]{\markboth{Chapter \thechapter.\ #1}{}}
%\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}
\fancyhf{} % reset all header and footer fields
\fancyhead[LE,RO]{\bfseries \thepage}
\fancyhead[LO]{\bfseries \nouppercase{\rightmark}}
\fancyhead[RE]{\bfseries \nouppercase{\leftmark}}
\renewcommand{\headrulewidth}{0.5pt}
\addtolength{\headheight}{1.6pt}
\fancypagestyle{plain}{
\fancyhf{}
\renewcommand{\headrulewidth}{0pt}
}


==> cesr_conversion.tex <==
%-----------------------------------------------%
% CesrTA Phase I Report - CESR Conversion       %
% Chapter coordinator:  Mark Palmer             %
% Page estimate:  85pp. total                   %
%-----------------------------------------------%
%!TEX root =  ../CesrTA_PhaseI_Report.tex

\chapter[The CESR Conversion]{The CESR Conversion to a Damping Ring Configuration}
\label{ch:cesr_conversion}

% Section - Overview of CESR Modifications
% Section coordinator - Mark Palmer
\input{CESR_Conversion/overview}

% Section - Vacuum System Modifications
% Section coordinator - Yulin Li
\input{CESR_Conversion/vacuum_system}

% Section - Electron Cloud Diagnostics
% Section coordinator - Mark Palmer
\input{CESR_Conversion/ec_diagnostics}

% Section - Beam Instrumentation and Feedback Upgrades
% Section coordinator - Mike Billing
\input{CESR_Conversion/beam_instrumentation}

% Section - General Accelerator Modifications and Upgrades
% Section coordinator - Mike Billing
\input{CESR_Conversion/general_modifications}


